$\rho - \omega$ Mixing in $J/\psi\to VP$ Decays

The study on $\rho-\omega$ mixing is mainly focused on vector mesons decay with isospin I=1, namely $\rho(\omega)\to\pi^+\pi^-$ process. In this paper, we present the study of $\rho-\omega$ mixing in $\rho(\omega)\to\pi^+\pi^-\pi^0$ (I=0) using a flavor parameterization model for $J/\psi\to VP$ process. By fitting theoretical frame to PDG data, we obtain the SU(3)-breaking effect parameters $s_V=0.03\pm 0.12,\ s_P=0.17\pm 0.17$ and the $\rho-\omega$ mixing polarization operator $\Pi_{\rho \omega}=0.006\pm 0.011\text{\text{GeV}}^2$. The branching ratios are also renewed when mixing effect is incorporated: $Br(J/\psi\to \omega\pi^0) = (3.64 \pm 0.37)\times 10^{-4}$, $Br(J/\psi\to \omega\eta) = (1.48 \pm 0.17)\times 10^{-3}$, $Br(J/\psi\to \omega\eta^{\prime}) = (1.55\pm 0.56)\times 10^{-4}$; they are different from the corresponding PDG2012 values by 19%, 15% and 15%, respectively.

==> charpters/TittleAbstract20130407.tex <==

\title{$\rho - \omega$ Mixing in $\jpsi\to VP$ Decays}
\author{...}
%\author{WANG Dong.$^{1,2}$, LI Gang$^{2}$, YUAN Changzheng$^{2}$, BAN Yong$^{1}$}
%\email[my e-mail]{ledong@pku.edu.cn}
%\homepage[peking homepage]{www.pku.edu.cn}
%\thanks{...}
%\altaffiliation[Also at ]{$^{1}$Peking University \  $^{2}$Institude of High Energy Physics.}{}
%\affiliation{Peking University, Institude of High Energy Physics}
%\email[my e-mail]{ledong@pku.edu.cn}
%\homepage[PK  homepage:]{www.pku.edu.cn}
%\homepage[IHEP homepage:]{www.ihep.ac.cn}
%\thanks{...}
%\date{November 22, 2011}
\date{\today}

\begin{abstract}
I review some resent ... in .... Many ... are applied to research on .... These .... In this paper, we present measurements of...
\end{abstract}




==> charpters/TittleAbstract20130605.tex <==
%\fancyhead[c]{\small Chinese Physics C~~~Vol. 37, No. 1 (2013)
%010201} \fancyfoot[C]{\small 010201-\thepage}
%
%\footnotetext[0]{Received 14 March 2009}

\title{$\rho - \omega$ Mixing in $\jpsi\to VP$ Decays \thanks{Supported by Ministry of Science and Technology of China (973 Project No. 2009CB825200)}}

\author{%
      WANG Dong$^{1}$%
\quad BAN Yong$^{1;1)}$\email{bany@pku.edu.cn}%
\quad LI Gang$^{2}$
}



\address{%
$^1$ School of Physics, State Key Laboratory of Nuclear Physics and Technology, Peking University,  Beijing 100871, China\\
$^2$ Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China\\
}

\begin{abstract}
The study on $\rho-\omega$ mixing is mainly focused on vector mesons decay with isospin $I=1$, namely $\rho(\omega)\to\pi^+\pi^-$ process. In this paper, we present the study of $\rho-\omega$ mixing in $\rho(\omega)\to\pi^+\pi^-\pi^0$ ($I=0$) using a flavor parameterization model for $J/\psi\to VP$ process. By fitting theoretical frame to PDG data, we obtain the SU(3)-breaking effect parameters $s_V=0.03\pm 0.12,\ s_P=0.17\pm 0.17$ and the $\rho-\omega$ mixing polarization operator $\Pi _{\rho \omega }=0.006\pm 0.011\text{ \text{GeV}}^2$. The branching ratios are also renewed when mixing effect is incorporated:
$Br(J/\psi\to \omega\pi^0) = (3.64 \pm 0.37)\times 10^{-4}$,
$Br(J/\psi\to \omega\eta)  = (1.48 \pm 0.17)\times 10^{-3}$,
$Br(J/\psi\to \omega\eta^{\prime}) = (1.55\pm 0.56)\times 10^{-4}$;
 they are different from the corresponding PDG2012 values by $19\%$, $15\%$ and $15\%$, respectively.
\end{abstract}

%\begin{keyword}
%$\rho-\omega$ mixing, branching ratio, $J/\psi\to VP$ decay.
%\end{keyword}

\begin{pacs}
12.39.-x,
12.40.Vv,
13.25.Gv
\end{pacs}

\maketitle

%\footnotetext[0]{\hspace*{-3mm}\raisebox{0.3ex}{$\scriptstyle\copyright$}2013
%Chinese Physical Society and the Institute of High Energy Physics
%of the Chinese Academy of Sciences and the Institute
%of Modern Physics of the Chinese Academy of Sciences and IOP Publishing Ltd}%


